Automated inference of production rules for glycans

Glycans are tree-like polymers made up of sugar monomer building blocks. They are found on the surface of all living cells, and distinct glycan trees act as identity markers for distinct cell types. Proteins called GTase enzymes assemble glycans via the successive addition of monomer building blocks. The rules by which the enzymes operate are not fully understood. In this paper, we present the first SMT-solver-based iterative method that infers the assembly process of the glycans by analyzing the set of glycans from a cell. We have built a tool based on the method and applied it to infer rules based on published glycan data.

==> related.tex <==
% Success of formal methods
Formal methods have successful in applications to a vast range of
problems from the analysis of
systems~\cite{biere1999symbolic2,biere2003bounded,lattice77,ClarkeCEGAR}.
Synthesis of programs that implements a given behavior
has been a focus of research for a while~\cite{PnueliSynthesis}.
In recent years, the synthesis of programs using SAT/SMT solvers
has gained momentum~\cite{SrivastavaSynthesis,Solar-Lezama2005,sygus}.
%
The approach encodes the search of a program that exhibits a certain
behavior into a satisfiability problem.
%
The solvers attempt to find a solution of the satisfiability problem.
%
The solution is the synthesized program.



% Boolean networks

% Program synthesis
Since the formal methods have been exhibiting effectiveness in the vast
range of problems, the
systems biology community has been applying the methods for various
biological problems~\cite{fisher2007executable}.
The key focus has been to model gene regulatory networks (GRNs)~\cite{wang2012BooleanOverview,delayedCTMC}.

There are many biological processes where we can observe the system behavior,
but the exact mechanisms of the processes are not known.
%
Recently, the methods for formal synthesis are finding their applications in biology~\cite{dunn2014defining,xuPluripotency,booleanModelKarp13,paoletti2014analyzing,koksal2013synthesis,fisher2015synthesising}.
%
As far as we know, there has been no similar computation based analysis of glycan production rules.


% In~\cite{},
% GRNs with unknown interactions are modeled using
% a automata-like model with missing components
% and the specification is the variations of the behavior of the system under mutations.
% Their approach uses a counterexample-guided inductive synthesis (CEGIS) based algorithm~\cite{cegis}.
% CEGIS is a framework for synthesis. It first finds a program that may satisfy `samples' from
% the specification. If the synthesized program satisfies the specifications, the CEGIS terminates.
% Otherwise, the method learns a new sample where the program violates the specifications.
% It adds the sample to the set and goes to the next iteration.
% Typically, the constraint solvers find the programs during intermediate steps of CEGIS by
% solving the generated queries.
% %
% Our method follows a similar pattern, where
% a set of sampled observations is a specification, i.e., output molecules,
% and we need to find the governing programs, i.e., production rules.
% %
% In a subsequent work~\cite{}, a Boolean network model is used,
% the functions attached to the nodes are considered unknown, and
% a different kind of data sets provides the behavior specification.
% In this approach, their earlier method is adopted to work in the new situation.
% %


%--------------------- DO NOT ERASE BELOW THIS LINE --------------------------

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

